Low Complexity Method for Simulation of Epidemics Based on Dijkstra's Algorithm

Models of epidemics over networks have become popular, as they describe the impact of individual behavior on infection spread. However, they come with high computational complexity, which constitutes a problem in case large-scale scenarios are considered. This paper presents a discrete-time multi-agent SIR (Susceptible, Infected, Recovered) model that extends known results in literature. Based on that, using the novel notion of Contagion Graph, it proposes a graphbased method derived from Dijkstra's algorithm that allows to decrease the computational complexity of a simulation. The Contagion Graph can be also employed as an approximation scheme describing the "mean behavior" of an epidemic over a network and requiring low computational power. Theoretical findings are confirmed by randomized large-scale simulation.

==> dynamics.tex <==
%!TEX root = journal.tex
% Suppose that, at time 
% $\bar{k}\in\natnum$, individual $i$
% contracts the disease and
% individual
% $j\neq i$ is susceptible.
% We define the recovery time
% of individual $i$ as an 
% a~priori-known constant
% $R_i\in\posint$; therefore,
% $i$ remains in the infected
% state
% until time $\bar{k}+R_i$, when
% it finally enters the 
% recovered state.
% For all
% $k\in\{\bar{k},\ldots,
% \bar{k}+R_i-1\}$, $j\in\neigh$
% has probability
% $p_{ij}(k)$ to contract the
% disease at time $k+1$ from $i$,
% and
% probability $1-p_{ij}(k)$
% to remain in the susceptible
% state.
% We model this behaviour by
% defining
% a random variable with
% Bernoulli
% distribution
% $\coeff\sim\mathcal{B}
% (p_{ij}(k))$ such that,
% $\forall i,j\in\nodes$,
% $\coeff=\coeff[j][i]$.
% Condition $\coeff=1$ indicates
% that individuals $i$ and $j$ 
% have an interaction at time $k$,
% such that, if one of them is
% infected and the other is susceptible,
% the susceptible one enters the
% infected state at time $k+1$.
% We associate, for every agent
% $i\in\nodes$:
% \begin{itemize}
%     \item the infection
%     state $x_i(k)\in\{0,1\}$,
%     which is 1 if $i$ is
%     infected at time $k$, 0
%     otherwise;
%     \item the
%     infection stopwatch 
%     $s_i(k)\in\{0,1,\ldots,R_i\}$,
%     which measures the number of
%     time steps
%     that have been occurred since
%     the moment $i$ contracted
%     the disease.
% \end{itemize}
% Then, the dynamics of each
% agent $i\in\nodes$ evolves
% according to the
% non-linear
% discrete-time system~\eqref{eq:system},
% where $\varrho:\real\mapsto\{0,1\}$
% is the step function
% \[
% \varrho(\circ) =
% \begin{cases}
%     0 & \mbox{ if }\circ\leq 0\\
%     1 & \mbox{ if }\circ>0
% \end{cases}.
% \]
% 
% %\begin{figure*}[htb]
% 	\begin{align}\label{eq:system}
% 	\begin{cases}
% 	x_i(k+1)
% 	&=
% 	\varrho
% 	(R_i-1-s_i(k))
% 	\varrho
% 	\left(
% 	x_i(k) + 
% 	\sum\limits_{j\in\neigh} 
% 	\coeff x_j(k)
% 	\right)
% 	\\
% 	s_i(k+1)
% 	&=
% 	s_i(k) 
% 	+ 
% 	x_i(k)
% 	\end{cases}
% 	\end{align}	
% %\end{figure*}
% 
% 
% 
% \zor{Maybe an example and some other words}


==> model_dynamics.tex <==
%!TEX root = journal.tex
% In this section, we state
% the dynamical equations that
% describe the spreading of the
% epidemics among individuals.
% The dynamics is based on the
% susceptible-infected-recovered
% (SIR) model.
% This means that, after an
% agent contracts the disease,
% it will
% eventually recover in finite
% time.
% Moreover, after an agent
% enters the recovered state,
% it can not be infected
% again.
% 
% \subsection{Dynamics}
% \input{dynamics}
% 
% \subsection{Contagion graph}
% \input{contagion_graph}

